High-dimensional Bayesian inference via the Unadjusted Langevin Algorithm

We consider in this paper the problem of sampling a high-dimensional probability distribution $\pi$ having a density with respect to the Lebesgue measure on $\mathbb{R}^d$, known up to a normalization constant $x \mapsto \pi(x)= \mathrm{e}^{-U(x)}/\int_{\mathbb{R}^d} \mathrm{e}^{-U(y)} \mathrm{d} y$. Such problem naturally occurs for example in Bayesian inference and machine learning. Under the assumption that $U$ is continuously differentiable, $\nabla U$ is globally Lipschitz and $U$ is strongly convex, we obtain non-asymptotic bounds for the convergence to stationarity in Wasserstein distance of order $2$ and total variation distance of the sampling method based on the Euler discretization of the Langevin stochastic differential equation, for both constant and decreasing step sizes. The dependence on the dimension of the state space of these bounds is explicit. The convergence of an appropriately weighted empirical measure is also investigated and bounds for the mean square error and exponential deviation inequality are reported for functions which are measurable and bounded. An illustration to Bayesian inference for binary regression is presented to support our claims.

==> MSE.tex <==
\section{Mean square error and concentration for Lipschitz functions}
\sectionmark{Mean square error and concentration for Lip. functions}
\label{sec:MSE}
Let $f : \rset^d \to \rset$ be a Lipschitz function and $(X_k)_{k \geq
  0}$ the Euler discretization of the Langevin diffusion. In this
section we study the approximation of $\int_{\rset^d} f(y) \pi(\rmd
y)$ by the weighted average estimator
\begin{equation}
 \label{eq:def_GammaN_plusn-new}
\hat{\pi}^N_n(f)= \sum_{k=N+1} ^{N+n} \weight{k} f(X_k) \eqsp, \quad  \weight{k}= \gamma_{k+1} \Gamma_{N+2 , N+n+1}^{-1}\eqsp.
 \end{equation}
where  $N \geq 0$ is the length of the burn-in period, $n \geq 1$ is the number of samples, and for $n,p \in \nset$, $\Gamma_{n,p}$ is given by \eqref{eq:def_Gamma}.
In all this section, $\PP_x$ and $\PE_x$ denote the probability and the expectation respectively, induced on $((\rset^{d})^{\nset}, \mathcal{B}(\rset^d)^{\nset})$ by the Markov chain $(X_n)_{n \geq 0}$ started at $x \in \rset^d$.
%\subsection*{Mean square error}
We first compute an explicit bound for the Mean Squared Error ($\MSE$) of this estimator defined by:
\begin{equation*}
%\label{eq:decomp_MSE}
\MSE_f^{N,n} = \expeMarkov{x}{\abs{\hat{\pi}_n^N(f)- \pi(f) }^2}  = \left\{ \PE_x[ \estimateur{f} ] - \pi(f) \right\}^2 + \VarDeux{x}{ \estimateur{f} }\eqsp.
\end{equation*}
%The MSE can be decomposed into the sum of the squared bias and the variance
%We bound separately these two terms.
We first  bound the bias. For all $k \in \{ N+1, \dots, N+n \}$, let $\xi_k$ be the optimal transference plan between $\delta_x Q_\gamma^k$ and $\pi$ for $W_2$, \ie~$W_2^2(\delta_x Q_\gamma^k,\pi) = \int_{\rset^d \times \rset^d} \norm[2]{x-y} \rmd\xi_k( x, y)$. Then by the Jensen inequality and because $f$ is Lipschitz, we have:
\begin{align*}
\defEns{\PE_x[\estimateur{f}]-\pi(f) }^2
&= \parenthese{\sum_{k=N+1} ^{N+n} \weight{k} \int_{\rset^d \times \rset^d} \{f(z) - f(y)\} \xi_k (\rmd z , \rmd y) }^2 \\
&\leq \norm{f}_{\Lip}^2  \sum_{k=N+1}^{N+n} \weight{k} \int_{\rset^d \times \rset^d}  \norm{z-y}^2 \xi_k (\rmd z , \rmd y) \eqsp.
\end{align*}
Let $(\gamma_k)_{k \geq 1}$ be a non-increasing sequence with $\gamma_1 \leq 1/(m+L)$ and recall that $x^\star$ is the unique minimizer of $U$. Using \Cref{theo:distance_Euler_diffusion} and \Cref{theo:distance_Euler_diffusionD}, we end up with the following bound:
\begin{equation}
\label{theo:bound_biasD}
\left\{ \PE_x[ \estimateur{f} ] - \pi(f) \right\}^2
\leq \norm{f}_{\Lip}^2  \sum_{k=N+1}^{N+n} \weight{k} \defEns{ ( \norm[2]{x-x^\star}+d/m)u_k^{(1)}(\gamma)+ w_k(\gamma)} \eqsp,
\end{equation}
where $u_n^{(1)}(\gamma)$ is given in \eqref{eq:def_u1} and $w_n(\gamma)$ is equal to $u_n^{(2)}(\gamma)$ defined by \eqref{eq:def_u2} if   \Cref{assum:regularity_2}-\Cref{assum:potentialU} hold, and to $u_n^{(3)}(\gamma)$, defined by \eqref{eq:def_u2D}, if  \Cref{assum:regularity_2}-\Cref{assum:potentialU} and \Cref{assum:reg_plus} hold.

% \begin{proposition}
% \label{theo:bound_bias}
% Assume \Cref{assum:regularity_2} and \Cref{assum:potentialU}. Let $(\gamma_k)_{k \geq 1}$ be a non-increasing sequence with $\gamma_1 \leq 1/(m+L)$. Let $x^\star$ be the unique minimizer of $U$. Let $(X_n)_{n \geq 0}$ be given by \eqref{eq:euler-proposal-2} and started at $x \in \rset^d$. Then for all $n,N \geq 0$ and Lipschitz function $f : \rset^d \to \rset$, $\norm{f}_{\Lip} \leq 1$:
% \begin{equation*}
% \left\{ \PE_x[ \estimateur{f} ] - \pi(f) \right\}^2
% \leq  \sum_{k=N+1}^{N+n} \weight{k} \defEns{2 ( \norm[2]{x-x^\star}+d/m)u_k^{(1)}(\gamma)+ w_k(\gamma)} \eqsp,
% \end{equation*}
% where $u_n^{(1)}(\gamma)$ is given in \eqref{eq:def_u1} and $w_n(\gamma)$ is equal to $u_n^{(2)}(\gamma)$ defined by \eqref{eq:def_u2} and to $u_n^{(3)}(\gamma)$, defined by \eqref{eq:def_u2D}, if \Cref{assum:reg_plus} holds.
% \end{proposition}
%
%\begin{proof}
%
%Finally, the conclusion follows from \Cref{theo:distance_Euler_diffusion}.
%\end{proof}
Consider now the variance term. To control this term, we adapt the proof of \cite[Theorem 2]{joulin:ollivier:2010} for homogeneous Markov chain to our inhomogeneous setting, and we have:
\begin{theorem}
\label{theo:var}
Assume \Cref{assum:regularity_2} and \Cref{assum:potentialU}.
Let $(\gamma_k)_{k \geq 1}$ be a non-increasing sequence with $\gamma_1 \leq 2/(m+L)$.
%Let $(X_n)_{n \geq 0} $ be given by \eqref{eq:euler-proposal-2} and started at $x \in \rset^d$.
Then for all $N \geq 0$, $ n \geq 1$ and Lipschitz functions $f : \rset^d \to \rset$, we get
$\VarDeuxLigne{x}{\hat{\pi}_n^N(f)} \leq  8 \kappa^{-2} \norm{f}_{\Lip}^2 \Gamma_{N+2,N+n+1}^{-1} v_{N,n}(\gamma)$,
where
\begin{equation}
\label{eq:def_u_n_3}
v_{N,n}(\gamma) \eqdef \defEns{1+\Gamma_{N+2,N+n+1}^{-1}(\kappa^{-1}+2/(m+L))} \eqsp.
%\sum_{k=1}^N \gamma_k \prod_{j=k+1}^N (1 - \kappa \gamma_j)  \eqsp.
\end{equation}
\end{theorem}
\begin{proof}
Our main tool is the
Gaussian Poincar{\'e} inequality \cite[Theorem~3.20]{boucheron:lugosi:massart:2013}
%(see also \cite[Theorem 4.1.1]{bakry:gentil:ledoux:2014})
which
% states that if $Z=(Z_1,\dots,Z_d)$ is a Gaussian vector with identity covariance matrix, then $\Var{g(Z)} \leq \norm{g}_{\Lip}^2$ for all Lipschitz function $g : \rset^d \to \rset$.
% For all $y\in \rset^d$ and $\gaStep >0$, the Gaussian Poincar{\'e} inequality
can be applied to $R_\gamma(y,\cdot)$ defined by \eqref{eq:definition-Rgamma},  noticing that  $R_\gamma(y,\cdot)$ is a Gaussian distribution  with
mean $y - \gamma \nabla U(y)$ and covariance matrix $2 \gamma \operatorname{I}_d$:
for all Lipschitz function $g : \rset^d \to \rset$
\begin{equation}
\label{lem:var_1-new}
 R_\gamma \defEns{ g(\cdot) - R_\gamma g(y)}^2(y)   \leq 2 \gamma  \norm{g}_{\Lip}^2 \eqsp.
\end{equation}
% \begin{lemma}
% \label{lem:var_1-new}
% Assume \Cref{assum:regularity_2}.
% Let $g : \rset^d \to \rset$ be a Lipschitz function. Then for all $\gamma >0$, $y \in \rset^d$,
% \[
% 0 \leq R_\gamma \defEns{ g(\cdot) - R_\gamma g(y)}^2(y)= \int R_\gamma(y,\rmd z) \defEns{ g(z) - R_\gamma g(y)}^2   \leq 2 \gamma  \norm{g}_{\Lip}^2 \eqsp.
% \]
% \end{lemma}
To go further, we decompose $\hat{\pi}_n^N(f)-\PE_x[\hat{\pi}_n^N(f)]$ as the sum of martingale increments,
% \begin{equation}
% \label{eq:decomposition-error}
% \hat{\pi}_n^N(f)- \PE_x[\hat{\pi}_n^N(f)]= \sum_{k=N}^{N+n-1} \left\{ \CPE[x]{\hat{\pi}_n^N(f)}{\mcg_{k+1}} - \CPE[x]{\hat{\pi}_n^N(f)}{\mcg_k} \right\} + \CPE[x]{\hat{\pi}_n^N(f)}{\mcg_N} - \PE_x[\hat{\pi}_n^N(f)] \eqsp,
% \end{equation}
\wrt~$(\mcg_n)_{n \geq 0}$, the natural filtration associated with Euler approximation $(X_n)_{n \geq 0}$, and we get
\begin{multline}
\label{eq:decomposition-variance-new}
\VarDeux{x}{\hat{\pi}_n^N(f)}= \sum_{k=N}^{N+n-1} \PE_x\left[ \parenthese{ \CPE[x]{\hat{\pi}_n^N(f)}{\mcg_{k+1}} - \CPE[x]{\hat{\pi}_n^N(f)}{\mcg_k}}^2\right] \\
+
\expeMarkov{x}{\parenthese{\CPE[x]{\hat{\pi}_n^N(f)}{\mcg_N} - \PE_x[\hat{\pi}_n^N(f)]}^2}\eqsp.
\end{multline}
Since $\hat{\pi}_n^N(f)$ is an additive functional, the martingale increment
$\CPE[x]{\hat{\pi}_n^N(f)}{\mcg_{k+1}}- \CPE[x]{\hat{\pi}_n^N(f)}{\mcg_k}$ has a simple expression.
For $k = N+n-1,\dots,N+1$, define backward in time the function
\begin{equation}
\label{eq:def_mart_f-new}
\martInc^N_{n,k}: x_k \mapsto \omega_{k,n}^N f(x_{k}) +R_{\gamma_{k+1}} \martInc^N_{n,k+1}( x_k ) \eqsp,
\end{equation}
where $\martInc_{n,N+n}^N : x_{N+n} \mapsto \martInc_{n,N+n}^N (x_{N+n}) =  \weight{N+n} f(x_{N+n})$. Denote finally
\begin{equation}
\label{eq:def_F_f-new}
\martIncF^{N}_{n}: x_N \mapsto R_{\gamma_{N+1}} \martInc^N_{n,N+1}(x_N)\eqsp.
\end{equation}
Note that for $k \in \{N,\dots,N+n-1\}$, by the Markov property,
\begin{equation}
\label{eq:relation_mart_var_cond-new}
\martInc^N_{n,k+1}(X_{k+1}) - R_{\gamma_{k+1}}\martInc^N_{n,k+1}(X_{k})= \CPE[x]{\hat{\pi}_n^N(f)}{\mcg_{k+1}} - \CPE[x]{\hat{\pi}_n^N(f)}{\mcg_k} \eqsp,
\end{equation}
and $\martIncF^N_{n}(X_N)= \CPE[x]{\hat{\pi}_n^N(f)}{\mcg_N}$.
With these notations, \eqref{eq:decomposition-variance-new} may be equivalently expressed as
\begin{align}
\nonumber
\VarDeux{x}{\hat{\pi}_n^N(f)}
 = \sum_{k=N}^{N+n-1} \PE_x\left[ R_{\gamma_{k+1}}\defEns{\martInc^N_{n,k+1}(\cdot)
 - R_{\gamma_{k+1}}\martInc^N_{n,k+1}(X_{k}) }^2 (X_k) \right]\\
\label{eq:decomposition-variance-alter-new}
  + \VarDeux{x}{\martIncF_n^N(X_{N})}  \eqsp.
\end{align}
Now for $k=N+n-1,\dots,N$, we will use the Gaussian Poincar{\'e} inequality \eqref{lem:var_1-new}
to the sequence of function $\martInc_{n,k+1}^N$
to prove that $x \mapsto R_{\gamma_{k+1}}\{\martInc^N_{n,k+1}(\cdot) - R_{\gamma_{k+1}}\martInc^N_{n,k+1}(x)\}^2(x)$ is uniformly bounded.
It is required to bound the Lipschitz constant of $\martInc_{n,k}^N$ .
%  For $k \in \defEns{N,\dots,N+n-1}$ and
% for all $y,z \in \rset^d$, we have
% \begin{equation}
%   \label{eq:fixed_x_N_Nplusk_mart}
% \abs{\martInc^N_{n,k+1}(y) -\martInc^N_{n,k+1}(z) } =  \left| \weight{k+1}\defEns{f(y) - f(z)}
% + \sum_{i=k+2}^{N+n} \weight{i} \defEns{Q^{k+2,i}_\gamma f(y) - Q^{k+2,i}_\gamma f(z)} \right| \eqsp.
% \end{equation}


\begin{lemma}
\label{coro:induction_function_mart-new}
Assume \Cref{assum:regularity_2} and \Cref{assum:potentialU}. Let $(\gamma_k)_{k \geq 1}$ be a non-increasing sequence
with $\gamma_1 \leq 2/(m+L)$. Let $N \geq 0$ and $n \geq 1$.
 Then for all $y \in \rset^d$,  Lipschitz function $f$ and $k\in \defEns{N,\dots,N+n-1}$,
\begin{equation*}
 R_{\gamma_{k+1}}\defEns{\martInc^N_{n,k+1}(\cdot) - R_{\gamma_{k+1}}\martInc^N_{n,k+1}(y) }^2 (y)
\leq 8   \gamma_{k+1}\norm[2]{f}_{\Lip} (\kappa\Gamma_{N+2,N+n+1})^{-2} \eqsp,
%2 \norm[2]{f}_{\Lip} \gamma_{k+1} \left(\sum_{i=k+1}^{N+n} \weight{i} \prod_{j=k+1}^i(1- \kappa \gamma_j)^{1/2} \right)^2 \eqsp,
 \end{equation*}
 where $\martInc^N_{n,k+1}$ is given by \eqref{eq:def_mart_f-new}.
\end{lemma}

\begin{proof}[Proof of \Cref{theo:var}]
By \eqref{eq:def_mart_f-new}, $\normLigne{\martInc^N_{n,k}}_{\Lip} \leq \sum_{i=k+1}^{N+n} \weight{i} \normLigne{Q_\gamma^{k+2,i}f}_{\Lip}$.
Using  \Cref{propo:contraction_Euler-new}, the bound $(1-t)^{1/2} \leq 1 - t/2$ for $t \in \ccint{0,1}$ and the definition of $\weight{i}$ given by \eqref{eq:def_GammaN_plusn}, we have
\begin{equation*}
\norm{\martInc^N_{n,k}}_{\Lip} \leq \norm{f}_{\Lip} \sum_{i=k+1}^{N+n} \weight{i} \prod_{j=k+2}^i (1- \kappa \gamma_j/2) \leq 2 \norm{f}_{\Lip}( \kappa \Gamma_{N+2,N+n+1} )^{-1} \eqsp.
% & \leq 2 \norm{f}_{\Lip}( \kappa \Gamma_{N+2,N+n+1} )^{-1} \sum_{i=k+1}^{N+n}  \defEns{\prod_{j=k+2}^i (1- \kappa \gamma_j/2) - \prod_{j=k+2}^{i+1} (1- \kappa \gamma_j/2)} \\
\end{equation*}
Finally, the proof follows from \eqref{lem:var_1-new}.
\end{proof}

Also to control the last term in right hand side of \eqref{eq:decomposition-variance-alter-new},
we need to control the variance of $\martIncF_n^N(X_N)$ under $\delta_x Q^N_\gamma$. But similarly to the sequence of functions $\martInc_{n,k}^N$,
$\martIncF_n^N$ is Lipschitz by \Cref{propo:contraction_Euler-new} by definition, see \eqref{eq:def_F_f-new}.
% since for all $y,z \in \rset^d$, we have
% \begin{equation}
% \label{eq:mart_n_0^N_dev}
% \abs{\martIncF_{n}^N(y) -\martIncF^{N}_{n}(z) } =  \abs{ \sum_{i=N+1}^{N+n} \weight{i} \defEns{Q^{N+1,i}_\gamma f(y) - Q^{N+1,i}_\gamma f(z) }}  \eqsp.
% \end{equation}
Therefore it suffices to find some bound for the variance of $g$ under $\delta_y Q_\gamma^{n,p}$ , for $g: \rset^d \to \rset$ a Lipschitz function, $y \in \rset^d$ and $\gamma >0$, which is done in \Cref{lem:var_2}.


\begin{corollary}
\label{coro:function_F}
Assume \Cref{assum:regularity_2} and \Cref{assum:potentialU}. Let $(\gamma_k)_{k \geq 1}$ be a non-increasing sequence
with $\gamma_1 \leq 2/(m+L)$.
Then for all Lipschitz function $f$ and $x \in \rset^d$, $\VarDeuxLigne{x}{\martIncF^N_n(X_N)}
\leq  8 \kappa^{-3} \norm{f}_{\Lip}^2  \Gamma_{N+2,N+n+1} ^{-2}$,
where $\martIncF^N_n$ is given by \eqref{eq:def_F_f-new}.
\end{corollary}
\begin{proof}
By \eqref{eq:def_F_f-new}  and \Cref{propo:contraction_Euler-new}, $\martIncF_n^N$ is Lipschitz function with $\normLigne{\martIncF^N_n}_{\Lip} \leq  \sum_{i=N+1}^{N+n} \weight{i} \normLigne{Q_\gamma^{N+1,i}f}_{\Lip}$.
Using  \Cref{propo:contraction_Euler-new}, the bound $(1-t)^{1/2} \leq 1 - t/2$ for $t \in \ccint{0,1}$ and the definition of $\weight{i}$ given by \eqref{eq:def_GammaN_plusn}, we have
\begin{equation*}
\norm{\martIncF^N_n}_{\Lip} \leq \norm{f}_{\Lip} \sum_{i=N+1}^{N+n} \weight{i} \prod_{j=N+2}^i (1- \kappa \gamma_j/2) \leq 2 \norm{f}_{\Lip}( \kappa \Gamma_{N+2,N+n+1} )^{-1} \eqsp.
 % \leq 2\norm{f}_{\Lip}( \kappa\Gamma_{N+2,N+n+1} )^{-1} \sum_{i=N+1}^{N+n}  \defEns{\prod_{j=N+2}^i (1- \kappa \gamma_j/2) - \prod_{j=N+2}^{i+1} (1- \kappa \gamma_j/2)} \\
\end{equation*}
The proof follows from \Cref{lem:var_2}.
\end{proof}
Plugging the bounds given by \Cref{coro:induction_function_mart-new} and \Cref{coro:function_F} in \eqref{eq:decomposition-variance-alter-new}, we have
\begin{align*}
\VarDeux{x}{\hat{\pi}_n^N(f)} &\leq  8 \kappa^{-2} \norm{f}_{\Lip}^2 \defEns{\Gamma_{N+2,N+n+1}^{-2} \Gamma_{N+1,N+n} + \kappa^{-1}\Gamma_{N+2,N+n+1}^{-2}} \\
&\leq 8\kappa^{-2} \norm{f}_{\Lip}^2 \defEns{\Gamma_{N+2,N+n+1}^{-1} + \Gamma_{N+2,N+n+1}^{-2}(\gamma_{N+1} + \kappa^{-1})} \eqsp.
\end{align*}
Using that $\gamma_{N+1} \leq 2/(m+L)$ concludes the proof.
\end{proof}


It is worth to observe that the bound for the variance is independent from the dimension.


We may now discuss the bounds on the MSE (obtained by combining the bounds for the squared bias \eqref{theo:bound_biasD} and the variance \Cref{theo:var}) for step sizes given for $k \geq 1$ by $\gamma_k = \gamma_1 k^{-\alpha}$ where $\alpha \in \ccint{0,1}$ and $\gamma_1 < 1/(m+L)$. Details of these calculations are postponed to \Cref{sapp:bound_MSE_strongly_convex}-\Cref{sapp:bound_MSE_strongly_convexD}.  The order of the bounds (up to numerical constants) of the MSE are summarized in \Cref{tab:bound_MSE_strongly_convex_fixe_gamma} as a function of  $\gamma_1$, $n$ and $N$. Note that in the infinite horizon setting, it is optimal to take $\alpha =1/2$ under \Cref{assum:regularity_2} and \Cref{assum:potentialU}, and $\alpha =1/3$ under \Cref{assum:regularity_2}, \Cref{assum:potentialU} and \Cref{assum:reg_plus}.
\begin{table}[h]
\centering
\begin{normalsize}
\begin{tabular}{|c|c|c|}
\hline
& Bound for the MSE\\
    \hline
    $\alpha =0$ & $\gamma_1 + (\gamma_1 n)^{-1}\defEns{1+\exp(-\kappa \gamma_1 N /2)}$ \\
\hline
$\alpha \in \ooint{0,1/2}$ &$\gamma_1n^{-\alpha} + (\gamma_1 n^{1-\alpha})^{-1}\defEns{1+\exp(-\kappa \gamma_1 N^{1-\alpha} /(2(1-\alpha)))}$\\
\hline
$\alpha =1/2$& $\gamma_1 \log(n) n^{-1/2} + (\gamma_1 n^{1/2})^{-1}\defEns{1+\exp(-\kappa \gamma_1 N^{1/2} /4)}$\\
\hline
 $\alpha \in \ooint{1/2,1}$& $n^{\alpha-1}\parentheseDeux{\gamma_1 + \gamma_1^{-1}\defEns{1+ \exp(-\kappa \gamma_1  N^{1-\alpha} /(2(1-\alpha)))}}$
\\
\hline
 $\alpha =1$& $\bigO(\log(n)^{-1})$ for $\gamma_1 > 2 \kappa^{-1}$
\\
\hline
\end{tabular}
\caption{\normalsize{Bound for the MSE for $\gamma_k = \gamma_1 k^{-\alpha}$ for fixed $\gamma_1$ and $N$ under \Cref{assum:regularity_2} and \Cref{assum:potentialU}}}
\label{tab:bound_MSE_strongly_convex_fixe_gamma}
\end{normalsize}
\end{table}
\begin{table}[h]
\centering
\begin{normalsize}
\begin{tabular}{|c|c|c|}
\hline
& Bound for the MSE\\
    \hline
    $\alpha =0$ & $\gamma_1^2 + (\gamma_1 n)^{-1}\{1+\exp(-\kappa \gamma_1 N /2)\}$ \\
\hline
$\alpha \in \ooint{0,1/3}$ &$\gamma_1^2n^{-2\alpha} + (\gamma_1 n^{1-\alpha})^{-1}\{1+\exp(-\kappa \gamma_1 N^{1-\alpha} /(2(1-\alpha)))\}$\\
\hline
$\alpha =1/3$& $\gamma_1^2 \log(n) n^{-2/3} + (\gamma_1 n^{2/3})^{-1}\{1+\exp(-\kappa \gamma_1 N^{1/2} /4)\}$\\
\hline
 $\alpha \in \ooint{1/3,1}$& $n^{\alpha-1}\parentheseDeux{\gamma_1^2 + \gamma_1^{-1}\{1+\exp(-\kappa \gamma_1  N^{1-\alpha} /(2(1-\alpha)))\}}$
\\
\hline
 $\alpha =1$& $\bigO(\log(n)^{-1})$ for $\gamma_1 > 4 \kappa^{-1}$
\\
\hline
\end{tabular}
\caption{\normalsize{Bound for the MSE for $\gamma_k = \gamma_1 k^{-\alpha}$ for fixed $\gamma_1$ and $N$ under \Cref{assum:regularity_2}, \Cref{assum:potentialU} and \Cref{assum:reg_plus}}}
\label{tab:bound_MSE_strongly_convex_fixe_gammaD}
\end{normalsize}
\end{table}

If the total number of iterations $n+N$ is held fixed (fixed horizon
setting), we may optimize the value of the
step size $\gamma_1$ but also of the burn-in period $N$ to minimize
the upper bound on the MSE.  The order (in $n$) for different values
of $\alpha \in \ccint{0,1}$ are summarized in
\Cref{tab:bound_MSE_fixed_horizon_strong_convex} (we display the order
in $n$ but not the constants, which are quite involved).

Let us discuss first the bounds based on
\Cref{theo:distance_Euler_diffusion}.  This time for any $\alpha \in
\coint{0,1/2}$, we can always achieve a MSE of order $n^{-1/2}$ by
choosing appropriately $\gamma_1$ and $N$ (for $\alpha =1/2$ we have
only $\log(n) n^{-1/2}$). For $\alpha \in \ocint{1/2,1}$, the best
strategy is to take $N=0$ and the largest possible value for $\gamma_1
= 1/(m+L)$, which leads to a MSE of order $n^{\alpha-1}$ for $\alpha
\in \ooint{0,1/2}$ and $\log(n)$ for $\alpha =1$.
% Finally, we note that from the explicit expression of the
% bound in \cite{durmus:moulines:2015:supplement}, that constant step
% sizes ($\alpha =0$) are  optimal. Finally, we mention that the bounds for $\alpha \in
% \coint{0,1/2}$ for a fixed number of iterations implies using the
% doubling trick (see \cite{hazan:kale:2014}) an anytime algorithm which
% guarantees for all $n \geq 1$, a MSE of order $\bigO(n^{-1/2})$.
We now discuss the bounds provided by \Cref{theo:distance_Euler_diffusionD}.
It appears that, for any $\alpha \in \coint{0,1/3}$, we
can always achieved the order $n^{-2/3}$ by choosing appropriately
$\gamma_1$ and $N$ (for $\alpha =1/3$ we have only $\log^{1/3}(n)
n^{-2/3}$).  The worst case is for $\alpha \in \ocint{1/3,1}$, where
in fact the best strategy is to take $N=0$ and the largest possible
value for $\gamma_1 = 1/(m+L)$.
%  Note that from the
% explicit expression of the bound in
% \cite[Section 5.2]{durmus:moulines:2015:supplement}, that constant step sizes
% ($\alpha =0$) are optimal again. Finally, we mention that the bounds for $\alpha \in
% \coint{0,1/3}$ for a fixed number of iterations implies using the
% doubling trick (see \cite{hazan:kale:2014}) an anytime algorithm which
% guarantees for all $n \geq 1$, a MSE of order $\bigO(n^{-2/3})$.

\begin{table}[h]
\centering
\begin{normalsize}
\begin{tabular}{|c|c|c|c|}
\hline
&\Cref{assum:regularity_2}, \Cref{assum:potentialU} and \Cref{assum:reg_plus}& \Cref{assum:regularity_2}, \Cref{assum:potentialU} and \Cref{assum:reg_plus}\\
    \hline
    $\alpha =0$ &  $n^{-1/2}$ &$ n^{-2/3}$\\
\hline
$\alpha \in \ooint{0,1/2}$ &$n^{-1/2}$& $n^{-2/3}$\\
\hline
$\alpha =1/2$  & $\log^{1/2}(n) n^{-1/2}$& $\log^{1/3}(n) n^{-2/3}$ \\
\hline
 $\alpha \in \ooint{1/2,1}$ &  $n^{\alpha-1}$ & $n^{\alpha-1}$
\\
\hline
\end{tabular}
\caption{Optimal bound for the MSE by choosing $\gamma_1$}
\label{tab:bound_MSE_fixed_horizon_strong_convex}
\end{normalsize}
\end{table}

It is worth to observe that the bound for the variance is independent from the dimension.


We may now discuss the bounds on the MSE (obtained by combining the bounds for the squared bias \eqref{theo:bound_biasD} and the variance \Cref{theo:var}) for step sizes given for $k \geq 1$ by $\gamma_k = \gamma_1 k^{-\alpha}$ where $\alpha \in \ccint{0,1}$ and $\gamma_1 < 1/(m+L)$. Details of these calculations are postponed to \Cref{sapp:bound_MSE_strongly_convex}-\Cref{sapp:bound_MSE_strongly_convexD}.  The order of the bounds (up to numerical constants) of the MSE are summarized in \Cref{tab:bound_MSE_strongly_convex_fixe_gamma} as a function of  $\gamma_1$, $n$ and $N$. Note that in the infinite horizon setting, it is optimal to take $\alpha =1/2$ under \Cref{assum:regularity_2} and \Cref{assum:potentialU}, and $\alpha =1/3$ under \Cref{assum:regularity_2}, \Cref{assum:potentialU} and \Cref{assum:reg_plus}.
\begin{table}[h]
\centering
\begin{normalsize}
\begin{tabular}{|c|c|c|}
\hline
& Bound for the MSE\\
    \hline
    $\alpha =0$ & $\gamma_1 + (\gamma_1 n)^{-1}\defEns{1+\exp(-\kappa \gamma_1 N /2)}$ \\
\hline
$\alpha \in \ooint{0,1/2}$ &$\gamma_1n^{-\alpha} + (\gamma_1 n^{1-\alpha})^{-1}\defEns{1+\exp(-\kappa \gamma_1 N^{1-\alpha} /(2(1-\alpha)))}$\\
\hline
$\alpha =1/2$& $\gamma_1 \log(n) n^{-1/2} + (\gamma_1 n^{1/2})^{-1}\defEns{1+\exp(-\kappa \gamma_1 N^{1/2} /4)}$\\
\hline
 $\alpha \in \ooint{1/2,1}$& $n^{\alpha-1}\parentheseDeux{\gamma_1 + \gamma_1^{-1}\defEns{1+ \exp(-\kappa \gamma_1  N^{1-\alpha} /(2(1-\alpha)))}}$
\\
\hline
 $\alpha =1$& $\bigO(\log(n)^{-1})$ for $\gamma_1 > 2 \kappa^{-1}$
\\
\hline
\end{tabular}
\caption{\normalsize{Bound for the MSE for $\gamma_k = \gamma_1 k^{-\alpha}$ for fixed $\gamma_1$ and $N$ under \Cref{assum:regularity_2} and \Cref{assum:potentialU}}}
\label{tab:bound_MSE_strongly_convex_fixe_gamma}
\end{normalsize}
\end{table}
\begin{table}[h]
\centering
\begin{normalsize}
\begin{tabular}{|c|c|c|}
\hline
& Bound for the MSE\\
    \hline
    $\alpha =0$ & $\gamma_1^2 + (\gamma_1 n)^{-1}\{1+\exp(-\kappa \gamma_1 N /2)\}$ \\
\hline
$\alpha \in \ooint{0,1/3}$ &$\gamma_1^2n^{-2\alpha} + (\gamma_1 n^{1-\alpha})^{-1}\{1+\exp(-\kappa \gamma_1 N^{1-\alpha} /(2(1-\alpha)))\}$\\
\hline
$\alpha =1/3$& $\gamma_1^2 \log(n) n^{-2/3} + (\gamma_1 n^{2/3})^{-1}\{1+\exp(-\kappa \gamma_1 N^{1/2} /4)\}$\\
\hline
 $\alpha \in \ooint{1/3,1}$& $n^{\alpha-1}\parentheseDeux{\gamma_1^2 + \gamma_1^{-1}\{1+\exp(-\kappa \gamma_1  N^{1-\alpha} /(2(1-\alpha)))\}}$
\\
\hline
 $\alpha =1$& $\bigO(\log(n)^{-1})$ for $\gamma_1 > 4 \kappa^{-1}$
\\
\hline
\end{tabular}
\caption{\normalsize{Bound for the MSE for $\gamma_k = \gamma_1 k^{-\alpha}$ for fixed $\gamma_1$ and $N$ under \Cref{assum:regularity_2}, \Cref{assum:potentialU} and \Cref{assum:reg_plus}}}
\label{tab:bound_MSE_strongly_convex_fixe_gammaD}
\end{normalsize}
\end{table}

If the total number of iterations $n+N$ is held fixed (fixed horizon
setting), we may optimize the value of the
step size $\gamma_1$ but also of the burn-in period $N$ to minimize
the upper bound on the MSE.  The order (in $n$) for different values
of $\alpha \in \ccint{0,1}$ are summarized in
\Cref{tab:bound_MSE_fixed_horizon_strong_convex} (we display the order
in $n$ but not the constants, which are quite involved).

Let us discuss first the bounds based on
\Cref{theo:distance_Euler_diffusion}.  This time for any $\alpha \in
\coint{0,1/2}$, we can always achieve a MSE of order $n^{-1/2}$ by
choosing appropriately $\gamma_1$ and $N$ (for $\alpha =1/2$ we have
only $\log(n) n^{-1/2}$). For $\alpha \in \ocint{1/2,1}$, the best
strategy is to take $N=0$ and the largest possible value for $\gamma_1
= 1/(m+L)$, which leads to a MSE of order $n^{\alpha-1}$ for $\alpha
\in \ooint{0,1/2}$ and $\log(n)$ for $\alpha =1$.
% Finally, we note that from the explicit expression of the
% bound in \cite{durmus:moulines:2015:supplement}, that constant step
% sizes ($\alpha =0$) are  optimal. Finally, we mention that the bounds for $\alpha \in
% \coint{0,1/2}$ for a fixed number of iterations implies using the
% doubling trick (see \cite{hazan:kale:2014}) an anytime algorithm which
% guarantees for all $n \geq 1$, a MSE of order $\bigO(n^{-1/2})$.
We now discuss the bounds provided by \Cref{theo:distance_Euler_diffusionD}.
It appears that, for any $\alpha \in \coint{0,1/3}$, we
can always achieved the order $n^{-2/3}$ by choosing appropriately
$\gamma_1$ and $N$ (for $\alpha =1/3$ we have only $\log^{1/3}(n)
n^{-2/3}$).  The worst case is for $\alpha \in \ocint{1/3,1}$, where
in fact the best strategy is to take $N=0$ and the largest possible
value for $\gamma_1 = 1/(m+L)$.
%  Note that from the
% explicit expression of the bound in
% \cite[Section 5.2]{durmus:moulines:2015:supplement}, that constant step sizes
% ($\alpha =0$) are optimal again. Finally, we mention that the bounds for $\alpha \in
% \coint{0,1/3}$ for a fixed number of iterations implies using the
% doubling trick (see \cite{hazan:kale:2014}) an anytime algorithm which
% guarantees for all $n \geq 1$, a MSE of order $\bigO(n^{-2/3})$.

\begin{table}[h]
\centering
\begin{normalsize}
\begin{tabular}{|c|c|c|c|}
\hline
&\Cref{assum:regularity_2}, \Cref{assum:potentialU} and \Cref{assum:reg_plus}& \Cref{assum:regularity_2}, \Cref{assum:potentialU} and \Cref{assum:reg_plus}\\
    \hline
    $\alpha =0$ &  $n^{-1/2}$ &$ n^{-2/3}$\\
\hline
$\alpha \in \ooint{0,1/2}$ &$n^{-1/2}$& $n^{-2/3}$\\
\hline
$\alpha =1/2$  & $\log^{1/2}(n) n^{-1/2}$& $\log^{1/3}(n) n^{-2/3}$ \\
\hline
 $\alpha \in \ooint{1/2,1}$ &  $n^{\alpha-1}$ & $n^{\alpha-1}$
\\
\hline
\end{tabular}
\caption{Optimal bound for the MSE by choosing $\gamma_1$}
\label{tab:bound_MSE_fixed_horizon_strong_convex}
\end{normalsize}
\end{table}




%\subsection*{Concentration inequalities}
We can also follow the proof of \cite[Theorem 5]{joulin:ollivier:2010} to establish an exponential deviation inequality for $\estimateur{f} - \PE_x[ \estimateur{f} ]$ given by \eqref{eq:def_GammaN_plusn}.


\begin{theorem}
\label{theo:concentration_gauss}
Assume \Cref{assum:regularity_2} and  \Cref{assum:potentialU}. Let $(\gamma_k)_{k \geq 1}$ be a non-increasing sequence with $\gamma_1 \leq 2/(m+L)$. Then for all $N \geq 0$, $n \geq 1$, $r>0$ and Lipschitz functions $f : \rset^d \to \rset$:
\begin{equation*}
 \probaMarkov{x}{\estimateur{f} \geq  \PE_x[ \estimateur{f} ]+r }\leq  \exp\left(  - \frac{r^2 \kappa ^2 \Gamma_{N+2, N+n+1}}{16 \norm{f}_{\Lip}^2 v_{N,n}(\gamma)}\right) \eqsp,
\end{equation*}
where $v_{N,n}(\gamma)$ is defined by \eqref{eq:def_u_n_3}.
\end{theorem}

\begin{proof}
Let  $N \geq 0$, $n \geq 1$, $x \in \rset^d$ and $f$ be a
Lipschitz function.
 To prove \Cref{theo:concentration_gauss}, we derive an upper bound of the Laplace transform of
$\estimateur{f} - \PE_x[ \estimateur{f} ]$. Consider the decomposition by martingale increments
\begin{multline*}
%\label{eq:link_lap_transf_mart_N_n_n}
\expeMarkov{x}{\rme^{\lambda \{ \estimateur{f} - \PE_x[ \estimateur{f} ] \}}}
 =  \expeMarkov{x}{\rme^{\lambda\{\CPE[x]{\hat{\pi}_n^N(f)}{\mcg_N} - \PE_x[\hat{\pi}_n^N(f)]\} + \sum_{k=N}^{N+n-1} \lambda  \{ \CPE[x]{\hat{\pi}_n^N(f)}{\mcg_{k+1}} - \CPE[x]{\hat{\pi}_n^N(f)}{\mcg_k} \} }} \eqsp.
\end{multline*}
Now using  \eqref{eq:relation_mart_var_cond-new} with the sequence of functions $(\martInc_{n,k}^N)$ and $\martIncF^N_n$ given by \eqref{eq:def_mart_f-new} and \eqref{eq:def_F_f-new}, respectively, we have by the Markov property
\begin{multline}
  \label{eq:link_lap_transf_mart_N_n_n}
\expeMarkov{x}{\rme^{\lambda \{ \estimateur{f} - \PE_x[ \estimateur{f} ] \}}}
%  &=\expeMarkov{x}{ \exp\parenthese{\lambda\{\martIncF_n^N(X_n)
%      -\expeMarkov{x}{\martIncF_n^N(X_n)}\} } \prod_{k=N}^{N+n-1} \CPE[x]{\exp \parenthese{
%      \lambda \{ D_{n,k+1}^N(X_k,X_{k+1}) \}}} {\mcg_{k}} }
\\
= \expeMarkov{x}{ \rme^{\lambda\defEns{\martIncF_n^N(X_n)
      -\expeMarkov{x}{\martIncF_n^N(X_n)}} } \prod_{k=N}^{N+n-1} R_{\gamma_{k+1}}\parentheseDeux{\rme^{
      \lambda \{ \martInc^N_{n,k+1}(\cdot) - R_{\gamma_{k+1}}\martInc^N_{n,k+1}(X_k) \} }}(X_k) } \eqsp,
\end{multline}
where $R_\gamma$ is given by \eqref{eq:definition-Rgamma} for $\gamma
>0$.
% and for $k \in \{N,\ldots,N+n-1\}$
% \begin{equation}
%   \label{eq:Ak}
% A_{k} =
% \end{equation}
 We use the same strategy to get concentration inequalities than
to bound the variance term in the previous section, replacing the
Gaussian Poincar{\'e} inequality by the log-Sobolev inequality to get
 uniform bound on $$
R_{\gamma_{k+1}}\{\exp ( \lambda
\lbrace \martInc^N_{n,k+1}( \cdot ) -
R_{\gamma_{k+1}}\martInc^N_{n,k+1}(X_{k}) \rbrace ) \}(X_k)$$
\wrt~$X_k$, for all $k \in \{N+1,\dots,N+n \}$.  Indeed for all $x \in \rset^d$ and $\gamma >0$, recall
that $R_\gamma(x,\cdot)$ is a Gaussian distribution with mean $x -
\gamma \nabla U(x)$ and covariance matrix $2 \gamma
\operatorname{I}_d$. The log-Sobolev inequality \cite[Theorem
5.5]{boucheron:lugosi:massart:2013} shows that for all Lipschitz
function $g :\rset^d \to \rset$, $x \in \rset^d$, $\gamma >0$ and
$\lambda >0$,
\begin{equation}
\label{lem:log_sob_R_gamma}
\int R_\gamma(x,\rmd y) \defEns{\exp\parenthese{\lambda \{g(y) - R_\gamma g(x) \}}} \leq \exp\parenthese{\gamma \lambda^2 \norm{g}_{\Lip}^2 } \eqsp.
\end{equation}
% \begin{lemma}[\protect{\cite[Theorem 5.5]{boucheron:lugosi:massart:2013}}]
% \label{lem:log_sob_R_gamma}
% Assume \Cref{assum:regularity_2}. Then for all Lipschitz function $g$, $\gamma >0$, $x \in \rset^d$ and $\lambda >0$,
% \[
% \int R_\gamma(x,\rmd y) \defEns{\exp\parenthese{\lambda \{g(y) - R_\gamma g(x) \}}} \leq \exp\parenthese{\gamma \lambda^2 \norm{g}_{\Lip}^2 } \eqsp.
% \]
% where $R_\gamma$ is given by \eqref{eq:definition-Rgamma}.
% \end{lemma}
We deduced from this result, \eqref{eq:relation_mart_var_cond-new} and  \Cref{propo:contraction_Euler-new}, an equivalent
of \Cref{coro:induction_function_mart-new} for the Laplace transform of
$\martInc^N_{n,k+1}$ under $\delta_y R_{\gamma_{k+1}}$ for $k \in \{N+1,\dots,N+n\}$ and all $y \in \rset^d$.

\begin{corollary}
\label{coro:lap_transf_mart}
Assume \Cref{assum:regularity_2} and \Cref{assum:potentialU}. Let $(\gamma_k)_{k \geq 1}$ be a non-increasing sequence with $\gamma_1 \leq 2/(m+L)$. Let $N \geq 0$ and $n \geq 1$. Then for all $k\in \defEns{N,\dots,N+n-1}$, $y \in \rset^d$ and $\lambda >0$,
\begin{equation*}
 R_{\gamma_{k+1}}\defEns{\rme^{
      \lambda \{ \martInc^N_{n,k+1}( \cdot ) -
      R_{\gamma_{k+1}}\martInc^N_{n,k+1}(y) \} }}(y)
 \leq \exp\parenthese{4  \gamma_{k+1}  \lambda^2 \norm{f}_{\Lip}^2 (\kappa \Gamma_{N+2,N+n+1})^{-2}} \eqsp,
\end{equation*}
where $\martInc_{n,k}^N$ is given by \eqref{eq:def_mart_f}.
% \begin{multline*}
% \int_{\rset^d} \rme^{ \lambda \martInc^N_{n,k+1}(\chunk{x}{N+1}{N+k+1})} R_{\gamma_{N+k+1}}(x_{N+k},\rmd x_{N+k+1} )\\
% \leq \exp\parenthese{  \lambda \martInc^N_{n,k}(\chunk{x}{N+1}{N+k}) +  \lambda^2 \norm{f}_{\Lip}^2    \gamma_{N+k+1} \left(\sum_{i=N+k+1}^{N+n} \weight{i} \exp\left( -(\kappa/2) \Gamma_{N+k+2,i} \right) \right)^2} \eqsp.
% \end{multline*}
% For all $x_N, \in \rset^d$,
% \begin{multline*}
% \int_{\rset^d}\rme^{\lambda \martInc^N_{n,1}(x_{N+1})}  R_{\gamma_{N+1}}(x_{N},\rmd x_{N+1} )\\
%  \leq \exp \parenthese{\lambda \martInc^N_{n,0}(x_N) + \lambda^2 \norm{f}_{\Lip}^2  (\Gamma^{N+1}_n)^{-2}  \gamma_{N+1} \left(\sum_{i=N+1}^{N+n} \gamma_i \exp\left( -(\kappa/2)\Gamma_{N+2,i}\right) \right)^2 }\eqsp,
% \end{multline*}
% where  $(\martInc^N_{n,k})_{k \in \defEns{0,\cdots,n}}$ are defined by
%   \eqref{eq:def_mart_f}.
\end{corollary}
It remains to control the Laplace
transform of $\martIncF_n^N$ under $\delta_x Q^N_\gamma$, where $\delta_x Q^N_\gamma$ is defined
by \eqref{eq:iterate_kernel}.  For this, using again that by
\eqref{eq:def_F_f-new} and
\Cref{propo:contraction_Euler-new},
$\martIncF_n^N$ is a Lipschitz function, we iterate \eqref{lem:log_sob_R_gamma}
to get bounds on the Laplace transform of Lipschitz function $g$ under
$Q^{n,\ell}_\gamma(y,\cdot)$ for all $y \in \rset^d$ and $n,\ell \geq 1$,
since for all $n,\ell \geq 1$, $Q^{n,\ell}_\gamma g$ is a Lipschitz function
by \Cref{propo:contraction_Euler-new}.

\begin{lemma}
\label{lem:transf_laplace_kernel}
Assume \Cref{assum:regularity_2} and \Cref{assum:potentialU}. Let $(\gamma_k)_{k \geq 1}$ be a non-increasing sequence with $\gamma_1 \leq 2/(m+L)$.  Let $g : \rset^d \to \rset$ be a Lipschitz function, then for all $n,p \geq 1$, $n \leq p$, $y \in \rset^d$ and $\lambda >0$:
\begin{equation}
\label{eq:induction-hypothesis}
Q^{n,p}_\gamma\defEns{\exp\parenthese{\lambda \{g(\cdot) -Q^{n,p}_\gamma g(y) \}}} (y) \leq
 \exp\left( \kappa^{-1}\lambda ^2 \norm{g}^2_{\Lip} \right) \eqsp,
\end{equation}
where $Q_{n,p}^\gamma$ is given by \eqref{eq:iterate_kernel}.
\end{lemma}

\begin{proof}
Let $(X_n)_{n \geq 0} $ the Euler approximation given by \eqref{eq:euler-proposal-2} and started at $y \in \rset^d$.
By decomposing $g(X_p)- \CPE[y]{g(X_p)}{\mcg_n}= \sum_{k=n+1}^p \{ \CPE[y]{g(X_p)}{\mcg_k} - \CPE[y]{g(X_p)}{\mcg_{k-1}} \}$,
and using $\CPE[y]{g(X_p)}{\mcg_k}=  Q_\gamma^{k+1,p} g(X_k)$, we get
\begin{align*}
&\CPE[y]{\exp\left(\lambda \defEns{g(X_p) - \CPE[y]{g(X_p)}{\mcg_n}} \right)}{\mcg_n} \\
&=  \CPE[y]{\prod_{k=n+1}^p\CPE[y]{\exp\left( \lambda \defEns{\CPE[y]{g(X_p)}{\mcg_k} - \CPE[y]{g(X_p)}{\mcg_{k-1}} }\right)}{\mcg_{k-1}} } {\mcg_n}\\
&= \CPE[y]{\prod_{k=n+1}^p R_{\gamma_k} \exp\left( \lambda\defEns{ Q_\gamma^{k+1,p} g(\cdot) -R_{\gamma_k} Q_\gamma^{k+1,p} g(X_{k-1})}\right) (X_{k-1})} {\mcg_n} \eqsp.
\end{align*}
By the Gaussian log-Sobolev inequality \eqref{lem:log_sob_R_gamma}, we get
\[
\CPE[y]{\exp\left(\lambda \defEns{g(X_p) - \CPE[y]{g(X_p)}{\mcg_n}} \right)}{\mcg_n} \leq \exp\left(\lambda^2 \sum_{k=n+1}^p \gamma_k \norm[2]{Q_\gamma^{k+1,p} g}_{\Lip} \right) \eqsp.
\]
 The proof follows from
\Cref{propo:contraction_Euler-new} and \Cref{lem:suite_recurrence_2}, using the bound $(1-t)^{1/2} \leq 1 - t/2$ for $t \in \ccint{0,1}$.

\end{proof}
Combining this result and $\normLigne{\martIncF^N_n}_{\Lip} \leq 2 \kappa^{-1} \norm{f}_{\Lip} \Gamma_{N+2,N+n+1}^{-1}$ by \Cref{propo:contraction_Euler-new}, we get an analogue of \Cref{coro:function_F} for the Laplace transform of $\martIncF^N_n$:
\begin{corollary}
\label{coro:lap_transf_F}
  Assume \Cref{assum:regularity_2} and \Cref{assum:potentialU}. Let
  $(\gamma_k)_{k \geq 1}$ be a non-increasing sequence with $\gamma_1
  \leq 2/(m+L)$. Let $N
  \geq 0$ and $n \geq 1$. Then for all $\lambda >0$ and $x \in \rset^d$,
  \begin{equation*}
  \expeMarkov{x}{ \rme^{\lambda\{\martIncF_n^N(X_n)
      -\expeMarkov{x}{\martIncF_n^N(X_n)}\} } }
\leq \exp\parenthese{4 \kappa^{-3}\lambda^2 \norm{f}_{\Lip}^2 \Gamma_{N+2,N+n+1}^{-2}}\eqsp,
 \end{equation*}
%\begin{multline*}
%  \expeMarkov{x}{ \rme^{\lambda\{\martIncF_n^N(X_n)
%      -\expeMarkov{x}{\martIncF_n^N(X_n)}\} } }
%    \\
%\leq \exp\parenthese{\lambda^2 \norm{f}_{\Lip}^2
%      \left(\sum_{i=N+1}^{N+n} \weight{i} \exp\left( -(\kappa/2) \Gamma_{N+2,i} \right) \right)^2
%      \sum_{k=1}^N \gamma_k  \exp \left( -\kappa\Gamma_{k+1,N} \right) }\eqsp,
% \end{multline*}
 where $\martIncF^N_{n}$ is given by \eqref{eq:def_F_f-new}.
\end{corollary}
 The Laplace transform of $\estimateur{f}$ can be explicitly bounded using \Cref{coro:lap_transf_mart} and \Cref{coro:lap_transf_F} in \eqref{eq:link_lap_transf_mart_N_n_n}.
\begin{proposition}
\label{lem:concentration_estimator}
Assume \Cref{assum:regularity_2} and \Cref{assum:potentialU}. Let $(\gamma_k)_{k \geq 1}$ be a non-increasing sequence with $\gamma_1 \leq 2/(m+L)$.  Then for all $N \geq 0$, $n \geq 1$, Lipschitz functions $f : \rset^d \to \rset$, $\lambda >0$ and $x \in \rset^d$:
\begin{equation*}
\expeMarkov{x}{\rme^{\lambda \{ \estimateur{f} - \PE_x[ \estimateur{f} ] \}}} \leq \exp \parenthese{ 4 \kappa^{-2} \lambda^2 \norm{f}_{\Lip}^2 \Gamma^{-1}_{N+2,N+n+1} u_{N,n}^{(3)}(\gamma) }
% \\
%  \times \exp \parenthese{\lambda^2  \norm{f}_{\Lip}^2  (\Gamma_n^N)^{-2}\sum_{k=0}^{n-1} \gamma_{N+n-k} \left(\sum_{i=N+n-k}^{N+n} \gamma_i \exp\left( -\sum_{l=N+n-k+1}^{i} \eta_l/2 \right) \right)^2} \\
% \times \exp \parenthese{\lambda^2 \norm{f}_{\Lip}^2  (\Gamma_n^N)^{-2} \left( \sum_{i=N+1}^{N+n} \gamma_i  \exp\left( -\sum_{l=N+n-k+1}^{i} \eta_l/2 \right)\right)^2 \sum_{k=1}^N \gamma_k \exp\left( -\sum_{i=k+1}^{N} \eta_i \right) }
\eqsp,
\end{equation*}
where  $u_{N,n}^{(3)}(\gamma)$ is  given by  \eqref{eq:def_u_n_3}.
\end{proposition}


\begin{proof}[Proof of \Cref{theo:concentration_gauss}]
  Using the Markov inequality and \Cref{lem:concentration_estimator}, for all $\lambda >0$, we have:
\begin{equation*}
\probaMarkov{x}{\estimateur{f} \geq  \PE_x[ \estimateur{f} ]+r }  \leq  \exp\left( -\lambda r +4 \kappa^{-2} \lambda^2 \norm{f}_{\Lip}^2 \Gamma^{-1}_{N+2,N+n+1} v_{N,n}(\gamma)    \right) \eqsp.
\end{equation*}
Then the result follows from taking $\lambda =  (r \kappa^2 \Gamma_{N+2,N+n+1}) /(8\norm{f}_{\Lip}^2  v_{N,n}(\gamma) )$.
\end{proof}

\end{proof}
%Similar to \Cref{theo:var}, the upper bound on the right hand side may be more conveniently expressed as follows
%\begin{corollary}
%\label{coro:concentration}
%Assume \Cref{assum:regularity_2} and \Cref{assum:potentialU}. Let $(\gamma_k)_{k \geq 1}$ be a non-increasing sequence with $\gamma_1 \leq 2/(m+L)$. Let $(X_n)_{n \geq 0}$ be given by \eqref{eq:euler-proposal-2} and started at $x \in \rset^d$. Then for all $N \geq 0$, $ n \geq 1$ and Lipschitz functions $f : \rset^d \to \rset$:
%\[
%\probaMarkov{x}{\estimateur{f} \geq  \PE_x[ \estimateur{f} ]+r} \leq  \exp\left(  -\frac{r^2 \Gamma_{N+1,N+n}}{8 \kappa^{-2} \norm{f}_{\Lip}^2(1+ \Gamma_{N+1,N+n}^{-1}C_3)}\right) \eqsp,
%\]
%where $8 \kappa^{-2}$ and $C_3$ are given by \eqref{eq:def_const_MSE}.
%\end{corollary}
%
%\begin{proof}
%The proof follows from \Cref{theo:concentration_gauss}, \eqref{eq:bound_u_3_n_var} and using that $\gamma_1 \leq 1/(m+L)$.
%\end{proof}
If we apply this result to the sequence $(\gamma_k)_{k \geq 1}$ defined for all $k \geq 1$ by $\gamma_k = \gamma_1 k^{-\alpha}$, for $\alpha \in \ccint{0,1}$, we end up with a concentration of order $\exp(-Cr^2 \gamma_1 n^{1-\alpha})$ for $\alpha \in \coint{0,1}$, for some constant $C \geq 0$ independent of $\gamma_1$ and $n$.





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main_supplement"
%%% End: 


==> header.tex <==


\usepackage[utf8]{inputenc}
\usepackage{amssymb}
\usepackage{makeidx}
\usepackage[english]{babel}
\usepackage{graphicx}
\usepackage{amsfonts,amsmath,amssymb,amsthm}
\usepackage{oldgerm}
\usepackage{mathrsfs}
\usepackage[active]{srcltx}
\usepackage{verbatim}
\usepackage{enumitem} %label option for enumerate \alph* \Alph* \roman* \Roman* or other... [label=$\bullet$], [label=\alph*]
%\usepackage[comma,authoryear,longnamesfirst]{natbib}
%\usepackage[authoryear]{natbib}
%\usepackage{enumerate}
\usepackage[toc,page]{appendix}
\usepackage{aliascnt,bbm}
\usepackage{bm}
\usepackage{array}
\usepackage[colorlinks = true, citecolor = blue]{hyperref}
%\usepackage[ruled,vlined]{algorithm2e}
\usepackage[textwidth=4cm,textsize=tiny]{todonotes}
\usepackage{xargs}
\usepackage{cellspace}
\usepackage{slashbox}


\usepackage[Symbolsmallscale]{upgreek}


\usepackage{accents}
\usepackage{dsfont}
\usepackage{aliascnt}
\usepackage{cleveref}
\makeatletter
\newtheorem{theorem}{Theorem}
\crefname{theorem}{theorem}{Theorems}
\Crefname{Theorem}{Theorem}{Theorems}


\newaliascnt{lemma}{theorem}
\newtheorem{lemma}[lemma]{Lemma}
\aliascntresetthe{lemma}
\crefname{lemma}{lemma}{lemmas}
\Crefname{Lemma}{Lemma}{Lemmas}

\newaliascnt{corollary}{theorem}
\newtheorem{corollary}[corollary]{Corollary}
\aliascntresetthe{corollary}
\crefname{corollary}{corollary}{corollaries}
\Crefname{Corollary}{Corollary}{Corollaries}

\newaliascnt{proposition}{theorem}
\newtheorem{proposition}[proposition]{Proposition}
\aliascntresetthe{proposition}
\crefname{proposition}{proposition}{propositions}
\Crefname{Proposition}{Proposition}{Propositions}

\newaliascnt{definition}{theorem}
\newtheorem{definition}[definition]{Definition}
\aliascntresetthe{definition}
\crefname{definition}{definition}{definitions}
\Crefname{Definition}{Definition}{Definitions}

\newaliascnt{remark}{theorem}
\newtheorem{remark}[remark]{Remark}
\aliascntresetthe{remark}
\crefname{remark}{remark}{remarks}
\Crefname{Remark}{Remark}{Remarks}


\newtheorem{example}[theorem]{Example}
\crefname{example}{example}{examples}
\Crefname{Example}{Example}{Examples}


\crefname{figure}{figure}{figures}
\Crefname{Figure}{Figure}{Figures}


\newtheorem{assumption}{\textbf{H}\hspace{-3pt}}
\Crefname{assumption}{\textbf{H}\hspace{-3pt}}{\textbf{H}\hspace{-3pt}}
\crefname{assumption}{\textbf{H}}{\textbf{H}}

\newtheorem{assumptionG}{\textbf{G}\hspace{-3pt}}
\Crefname{assumptionG}{\textbf{G}\hspace{-3pt}}{\textbf{G}\hspace{-3pt}}
\crefname{assumptionG}{\textbf{G}}{\textbf{G}}


\newtheorem{assumptionAR}{\textbf{AR}\hspace{-3pt}}
\Crefname{assumptionAR}{\textbf{AR}\hspace{-3pt}}{\textbf{AR}\hspace{-3pt}}
\crefname{assumptionAR}{\textbf{AR}}{\textbf{AR}}

\newenvironment{enumerateList}{ \begin{enumerate}[label=(\roman*),wide=0pt, labelindent=\parindent]}{\end{enumerate}}


%\usepackage[a4paper]{geometry} % required for statsoc+pdflatex


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> proof.tex <==
\section{Proofs}
\label{sec:proof}
% \subsection{Proof of  \Cref{theo:convergence-WZ-strongly-convex}}
% \label{proof:theo:convergence-WZ-strongly-convex}

% \begin{enumerate}[label=(\roman*), wide=0pt, labelindent=\parindent]
% \item
% The generator $\generator$ associated with $(P_t)_{t \geq 0}$ is given,
% for all $f \in C^2(\rset^d)$ and $x \in \rset^d$, by:
% \begin{equation}
% \label{eq:def_generator}
%   \generator f(x) = -\ps{\nabla U(x)}{\nabla f(x)} + \Delta f(x) \eqsp.
% \end{equation}
% Denote for all $x \in \rset^d$ by $\VStar(x) = \norm{x - x^\star}^2$.
% Under \Cref{assum:regularity_2}  $\sup_{t \in \ccint{0,T}} \PE_{x}[\norm[2]{Y_t^{}}] < \plusinfty$  for all $T \geq 0$. Therefore, the process $\parenthese{\VStar(Y_t) -\VStar(x) - \int_0 ^t \generator \VStar(Y_s) \rmd s}_{ t \geq 0}$
% is a $(\mathcal{F}_t)_{ t \geq 0}$-martingale under $\PP_x$.
% Since $\nabla U(x ^\star) = 0$ and using \eqref{eq:convex_forte_contra2}, we have
% \begin{equation}
% \label{eq:generator}
% \generator \VStar(x) = 2 \parenthese{ - \ps{\nabla U(x)- \nabla U(x^\star)}{x-x^{\star}} +d } \leq 2  \parenthese{ -m \VStar(x) +d } \eqsp.
% \end{equation}
% Denote for all $t \geq 0$ and $x \in \rset^d$ by $v(t,x) = P_t \VStar(x)$. Then we have,
% $\partial v(t,x)/\partial t = P_t \generator \VStar(x)$. Using \eqref{eq:generator}, we get
% \[
% \frac{\partial v(t,x)}{\partial t} = P_t \generator \VStar(x)  \leq  -2m P_t \VStar(x) + 2d = -2m v(t,x) + 2d \eqsp,
% \]
% and the proof follows from the Gr\"onwall inequality.
% \item Set $\VStar(x) = \norm[2]{x-x^\star}$. By Jensen's inequality and \Cref{lem:moment_diffusion}-\ref{item:moment_diffusion_2},  for all $c > 0$ and $t > 0$, we get
% \begin{align*}
% \pi(\VStar \wedge c)
% &= \pi P_t (\VStar \wedge c) \leq \pi (P_t \VStar \wedge c) = \int \pi(\rmd x)\, c \wedge \left\{ \|x-x^*\|^2 \rme^{-2 m t} + \frac{d}{m} (1-\rme^{-2mt})  \right\} \\
% &\leq \pi(\VStar \wedge c)  \rme^{-2 mt} + (1- \rme^{-2 mt}) d/m \eqsp.
% \end{align*}
% Taking the limit as $t \to \plusinfty$, we get $\pi(\VStar \wedge c) \leq d/m$.
% Using the monotone convergence theorem and taking the limit as $c \to \plusinfty$ concludes the proof.
% \end{enumerate}





\subsection{Proof of \Cref{theo:distance_Euler_diffusion} }
\label{sec:proof:theo:distance_Euler_diffusion}
We preface the proof by two technical Lemmata.
\begin{lemma}
\label{lem:moment_diffusion}
Let $(Y_t)_{t \geq 0}$ be the solution of \eqref{eq:langevin_2}
started at $x \in \rset^d$. For all $t \geq 0$ and $x \in \rset^d$,
\begin{equation*}
\expeMarkov{x}{\norm[2]{Y_t-x}} \leq  d t(2+L^2 t^2/3) + (3/2) t^2 L^2 \norm[2]{x-x^\star}  \eqsp.
\end{equation*}
\end{lemma}
\begin{proof}
Let $\generator$ be the generator associated with $(P_t)_{t \geq 0}$ defined by \eqref{eq:generator}.
  Denote for all $x,y \in \rset^d$, $\tilde{V}_x(y) = \norm[2]{y-x}$.  Note that the process $(\tilde{V}_x(Y_t^{}) -\tilde{V}_x(x) - \int_0 ^t \generator \tilde{V}_x(Y^{}_s) \rmd s)_{ t \geq 0}$,
is a $(\mathcal{F}_t)_{ t \geq 0}$-martingale under $\mathbb{P}_{x}$. Denote for all $t \geq
0$ and $x \in \rset^d$ by $\tilde{v}(t,x) = P_t \tilde{V}_x(x)$. Then we get,
\begin{equation}
\label{eq:Dynkin0_2}
\frac{\partial \tilde{v}(t,x)}{\partial t} = P_t \generator \tilde{V}_x(x) \eqsp.
\end{equation}
By \Cref{assum:potentialU}, we have for all $y \in \rset^d$, $\ps{\nabla U(y) - \nabla U(x)}{y-x} \geq m\norm[2]{x-y}$, which implies
\begin{equation*}
%\label{eq:generator_2}
\generator \tilde{V}_x(y) = 2 \parenthese{ - \ps{\nabla U(y)}{y-x} +d }
\leq 2  \parenthese{ -m \tilde{V}_x(y) +d - \ps{\nabla U(x) } {y-x}} \eqsp.
\end{equation*}
Using \eqref{eq:Dynkin0_2}, this inequality and that $\tilde{V}_x$ is positive, we get
\begin{equation}
\label{eq:preparation_Grown}
\frac{\partial \tilde{v}(t,x)}{\partial t} = P_t \generator \tilde{V}_x(x)   \leq 2\parenthese{ d -
  \int_{ \rset^d}  \ps{\nabla U(x) } {y-x} P_t( x , \rmd y)}  \eqsp.
\end{equation}
By the Cauchy-Schwarz inequality, $\nabla U( x ^\star) = 0$, \eqref{eq:langevin_2} and the Jensen inequality, we have,
\begin{align*}
&\abs{\expeMarkov{x}{ \ps{\nabla U(x) } {Y_t^{}-x}}} \leq \norm{\nabla U(x) } \norm{\expeMarkov{x}{Y_t^{}-x}}\\
& \quad \leq \norm{\nabla U(x)} \norm{\expeMarkov{x}{\int_0^t \left\{ \nabla U(Y_s^{}) - \nabla U(x^\star) \right\} \rmd s}} \\
&\quad \leq \sqrt{t} \norm{\nabla U(x)- \nabla U(x^\star) } \parenthese{ \int_0^t\PE_{x}\left[ \norm[2]{\nabla U(Y_s^{}) - \nabla U(x^\star) }\right]\rmd s }^{1/2}  \eqsp.
\end{align*}
Furthermore, by \Cref{assum:regularity_2} and \Cref{theo:convergence-WZ-strongly-convex}-\ref{item:moment_diffusion_2}, we have
\begin{align}
\nonumber
&\abs{\int_{ \rset^d}  \ps{\nabla U(x) } {y-x} P_t( x , \rmd y)} \leq  \sqrt{t} L^2 \norm{x-x^\star } \parenthese{\int_0^t\mathbb{E}_{x}\left[ \norm[2]{Y_s^{}-x^\star }\right]\rmd s}^{1/2}  \\
\nonumber
 &\qquad \qquad \leq  \sqrt{t}L^2 \norm{x-x^\star } \left(  \frac{1-\rme^{-2mt}}{2m} \norm[2]{x-x^\star} + \frac{2tm + \rme^{-2mt}-1}{2m} (d/m) \right)^{1/2} \\
\nonumber
%\label{eq:preparation_Grown_2}
&\qquad \qquad \leq  L^2 \norm{x-x^\star }  ( t \norm{x- x^{\star}} + t^{3/2} d^{1/2})\eqsp, \phantom{qfsdq}
\end{align}
where we used for the last line that by the Taylor theorem with remainder term, for all $s \geq 0 $, $(1-\rme^{-2ms})/(2m) \leq s$ and $(2ms+\rme^{-2ms}-1)/(2m) \leq m s^2$, and the inequality $\sqrt{a+b} \leq \sqrt{a} + \sqrt{b}$. Plugging this upper bound in \eqref{eq:preparation_Grown}, and since $ 2\norm{x-x^\star } t^{3/2} d^{1/2} \leq  t \norm[2]{x-x^\star} + t^2 d $, we get
\[
\frac{\partial \tilde{v}(t,x)}{\partial t} \leq   2d + 3 L^2 t \norm[2]{x-x^\star } + L^2t^{2} d
\]
Since $\tilde{v}(0,x) = 0$, the proof is completed by integrating this result.
\end{proof}
Let $(\filtration_t)_{t \geq 0}$ be the
filtration associated with $(B_t)_{t \geq 0}$ and $(Y_0,\overline{Y}_0)$.
\begin{lemma}
\label{lem:distance_Euler_diffusion_part1}
Assume \Cref{assum:regularity_2} and \Cref{assum:potentialU}. Let $(\gamma_k)_{k \geq 1}$
be a non-increasing sequence with $\gamma_1 \leq 1/(m+L)$.
Let $\zeta_0 \in \Pens_2(\rset^d \times \rset^d)$, $(Y_t,\overline{Y}_t)_{t \geq 0}$ such that $(Y_0, \overline{Y}_0)$ is distributed according to $\zeta_0$ and
given by \eqref{eq:definition_couplage_2}.  Then almost surely for all $n \geq 0$ and $\epsilon >0$,
\begin{align}
\label{eq:as_ineq1}
&\norm{Y_{\Gamma_{n+1}}- \overline{Y}_{\Gamma_{n+1}}}^2 \leq  \defEns{1- \gamma_{n+1}\left(\kappa-2\epsilon\right)} \norm{Y_{\Gamma_{n}}- \overline{Y}_{\Gamma_{n}}}^2
\\
\nonumber
&\qquad \qquad \qquad + (2 \gamma_{n+1}+(2 \epsilon)^{-1}) \int_{\Gamma_n}^{\Gamma_{n+1}}\norm{ \nabla U(Y_s) - \nabla U(Y_{\Gamma_n})}^2 \rmd s  \eqsp, \\
\label{eq:CPE_ineq1}
&\CPE{\norm{Y_{\Gamma_{n+1}}- \overline{Y}_{\Gamma_{n+1}}}^2}{{\filtration_{\Gamma_n}}}
\leq \defEns{1- \gamma_{n+1}\left(\kappa-2\epsilon\right)} \norm{Y_{\Gamma_{n}}- \overline{Y}_{\Gamma_{n}}}^2 \\
\nonumber
&  +  L^2\gamma_{n+1}^2 (1/(4\epsilon) +  \gamma_{n+1})\left(2 d +L^2\gamma_{n+1} \norm[2]{Y_{\Gamma_n}-x^\star} + dL^2 \gamma_{n+1}^2/6 \right) \eqsp.
\end{align}
\end{lemma}
\begin{proof}
Let $n \geq 0$ and $\epsilon >0$, and set $\Theta_n= Y_{\Gamma_{n}}- \overline{Y}_{\Gamma_{n}}$. We first show \eqref{eq:as_ineq1}.
By definition we have:
\begin{multline}
\label{eq:02/01}
\norm{\Theta_{n+1}}^2 =
 \norm{\Theta_n}^2+ \norm{ \int_{\Gamma_n}^{\Gamma_{n+1}}\defEns{ \nabla U(Y_s) - \nabla U(\overline{Y}_{\Gamma_{n}})} \rmd s}^2 \\- 2 \gamma_{n+1}\ps{\Theta_n}{\nabla U(Y_{\Gamma_n}) - \nabla U(\overline{Y}_{\Gamma_{n}})  } - 2 \int_{\Gamma_n}^{\Gamma_{n+1}}  \ps{\Theta_n}{\defEns{\nabla U(Y_s) - \nabla U(Y_{\Gamma_n})}} \rmd s   \eqsp.
\end{multline}
Young's inequality and  Jensen's inequality  imply
\begin{multline*}
 \norm{ \int_{\Gamma_n}^{\Gamma_{n+1}}\defEns{ \nabla U(Y_s) - \nabla U(\overline{Y}_{\Gamma_{n}}) } \rmd s}^2
%\label{eq:distance_diffusion_first_part_third_estimate}
\leq 2 \gamma_{n+1}^2 \norm{\nabla U ( Y_{\Gamma_n})- \nabla U(\overline{Y}_{\Gamma_{n}})}^2\\ +  2\gamma_{n+1} \int_{\Gamma_n}^{\Gamma_{n+1}}\norm{ \nabla U(Y_s) - \nabla U(Y_{\Gamma_n})}^2 \rmd s \eqsp.
\end{multline*}
Using \eqref{eq:convex_forte_contra1},  $\gamma_1 \leq 1/(m+L)$ and $(\gamma_k)_{k \geq 1}$ is non-increasing, \eqref{eq:02/01} becomes
\begin{align}
\nonumber
  \norm{\Theta_{n+1}}^2 \leq
 \defEns{1-\gamma_{n+1} \kappa } \norm{\Theta_n}^2+  2\gamma_{n+1} \int_{\Gamma_n}^{\Gamma_{n+1}}\norm{ \nabla U(Y_s) - \nabla U(Y_{\Gamma_n})}^2 \rmd s  \\
  \label{eq:002/01}
- 2 \int_{\Gamma_n}^{\Gamma_{n+1}}  \ps{\Theta_n}{\defEns{\nabla U(Y_s) - \nabla U(Y_{\Gamma_n})}} \rmd s   \eqsp.
\end{align}
%where we used \eqref{eq:convex_forte_contra2} in the last line.
Using the  inequality $|\ps{a}{b}| \leq \epsilon \|a\|^2 + (4 \epsilon)^{-1} \|b\|^2$  concludes the proof of \eqref{eq:as_ineq1}.

 We now prove \eqref{eq:CPE_ineq1}. Note that \eqref{eq:as_ineq1} implies that
\begin{multline}
\label{eq:distance_diffusion_first_part_fourth_estimate}
\CPE{\norm{\Theta_{n+1}}^2}{\filtration_{\Gamma_n}} \leq
 \defEns{1-\gamma_{n+1} (\kappa-2\epsilon) } \norm{\Theta_n}^2 \\
 +(2 \gamma_{n+1}+(2 \epsilon)^{-1}) \int_{\Gamma_n}^{\Gamma_{n+1}} \CPE{\norm{ \nabla U(Y_s) - \nabla U(Y_{\Gamma_n})  }^2}{\filtration_{\Gamma_n}} \rmd s \eqsp.
\end{multline}
By \Cref{assum:regularity_2}, the Markov property of $(Y_t)_{t \geq 0}$ and \Cref{lem:moment_diffusion}, we have
\begin{multline*}
\nonumber
\int_{\Gamma_n}^{\Gamma_{n+1}} \CPE{\norm{  \nabla U(Y_s) - \nabla U(Y_{\Gamma_n})  }^2}{\filtration_{\Gamma_n}} \rmd s %&
%\leq L^2\int_{\Gamma_n}^{\Gamma_{n+1}} \CPE{\norm{Y_s - Y_{\Gamma_n}}^2 }{\filtration_{\Gamma_n}} \rmd s\\
%\label{eq:distance_diffusion_first_part_second_estimate}
%\nonumber
%&
%\qquad \qquad \qquad
\\
 \leq L^2 \left( d \gamma_{n+1}^2 + dL^2 \gamma_{n+1}^4 /12+ (1/2)L^2 \gamma_{n+1}^3 \norm[2]{Y_{\Gamma_n}-x^\star}\right) \eqsp.
\end{multline*}
The proof is then concluded plugging this bound   in \eqref{eq:distance_diffusion_first_part_fourth_estimate} .
\end{proof}














\subsection{Proofs of \Cref{theo:distance_Euler_diffusionD}}
\label{sec:proof:distance_Euler_diffusionD}

\begin{lemma}
\label{lem:distance_Euler_diffusion_part1D}
Assume \Cref{assum:regularity_2}, \Cref{assum:potentialU} and \Cref{assum:reg_plus}. Let $(\gamma_k)_{k \geq 1}$
be a non-increasing sequence with $\gamma_1 \leq 1/(m+L)$.
and  $\zeta_0 \in \Pens_2(\rset^d \times \rset^d)$. Let $(Y_t,\overline{Y}_t)_{t \geq 0}$ be defined by \eqref{eq:definition_couplage_2} such that $(Y_0, \overline{Y}_0)$ is distributed according to $\zeta_0$. Then for all $n \geq 0$ and $\epsilon >0$, almost surely
\begin{align}
\nonumber
&\CPE{\norm[2]{Y_{\Gamma_{n+1}}- \overline{Y}_{\Gamma_{n+1}}}}{{\filtration_{\Gamma_n}}}
\leq \defEns{1- \gamma_{n+1}\left(\kappa-2\epsilon\right)} \norm{Y_{\Gamma_{n}}- \overline{Y}_{\Gamma_{n}}}^2  \\
\nonumber
& \phantom{aaaaaaaaaaaaaa}
+ \gamma_{n+1}^3\left\lbrace d(2L^2+ \epsilon^{-1}(d \tilde{L}^2/12 + \gamma_{n+1}L^4/4) + \gamma_{n+1}^2 L^4 /6 ) \right.\\
\nonumber
& \phantom{aaaaaaaaaaaaaaaaaaaaaaaaa} \left. +
L^4(\epsilon^{-1}/3+\gamma_{n+1}) \norm[2]{Y_{\Gamma_n}-\xstar} \right\rbrace \eqsp.
% +   L^2\gamma_{n+1}^3 \left(2 d +L^2\gamma_{n+1} \norm[2]{Y_{\Gamma_n}-x^\star} + dL^2 \gamma_{n+1}^2/6 \right)\\
% + (2 L^4 \gamma_{n+1}^3/3)\norm[2]{Y_{\Gamma_n}-\xstar} + L^4 d \gamma_{n+1}^4/2 +  \gamma_{n+1}^3 d \tilde{L}^2/6
%  \eqsp.
\end{align}
\end{lemma}
\begin{proof}
Let $n \geq 0$ and $\epsilon >0$, and set $\Theta_n= Y_{\Gamma_{n}}- \overline{Y}_{\Gamma_{n}}$.
Using Itô's formula, we have for all $s \in \coint{\Gamma_n,\Gamma_{n+1}}$,
\begin{align}
\nonumber
  \nabla U(Y_s) - \nabla U(Y_{\Gamma_n}) = \int_{\Gamma_n}^s \defEns{\nabla^2 U(Y_u) \nabla U(Y_u) + \vec{\Delta} (\nabla U) (Y_u)} \rmd u \\
\label{eq:ito-D}
+ \sqrt{2}\int_{\Gamma_n}^s \nabla^2 U(Y_u) \rmd B_u \eqsp.
\end{align}
Since $\Theta_n$ is $\filtration_{\Gamma_n}$-measurable and $(\int_{0}^s \nabla^2 U(Y_u) \rmd B_u)_{s \in \ccint{0,\Gamma_{n+1}}}$ is a $(\mcf_{s})_{s \in \ccint{0,\Gamma_{n+1}}}$-martingale under \Cref{assum:regularity_2}, by \eqref{eq:ito-D} we have:
\begin{multline*}
  \abs{\CPE{\ps{\Theta_n}{\nabla U(Y_s) - \nabla U(Y_{\Gamma_n})}} {\filtration_{\Gamma_n}} } \\
 =  \abs{\ps{\Theta_n}{\CPE{\int_{\Gamma_n}^s \defEns{\nabla^2 U(Y_u) \nabla U(Y_u) + \vec{\Delta} (\nabla U) (Y_u)} \rmd u}{\filtration_{\Gamma_n}}}}
\end{multline*}
Combining this equality and  $|\ps{a}{b}| \leq \epsilon \|a\|^2 + (4 \epsilon)^{-1} \|b\|^2$ in  \eqref{eq:002/01}  we have
\begin{align}
\nonumber
&\CPE{\norm{\Theta_{n+1}}^2}{\filtration_{\Gamma_n}} \leq \defEns{1-\gamma_{n+1} (\kappa-2\epsilon) } \norm{\Theta_n}^2 ++ (2\epsilon)^{-1}A \\
\label{eq:distance_diffusion_part1_first_estimateD}
%\nonumber
& \qquad \qquad \qquad \qquad 2\gamma_{n+1} \CPE{\int_{\Gamma_n}^{\Gamma_{n+1}}\norm{ \nabla U(Y_s) - \nabla U(Y_{\Gamma_n})}^2 \rmd s}{\filtration_{\Gamma_n}}
 \eqsp,
% &\qquad \qquad
% +\CPE{\norm{ \int_{\Gamma_n}^{\Gamma_{n+1}} \defEns{ \nabla U(Y_s) - \nabla U(\overline{Y}_{\Gamma_{n}})} \rmd s}^2 }{\filtration_{\Gamma_n}}  \eqsp.
\end{align}
where
\begin{equation*}
%  \label{eq:def_A_proof}
  A =  \int_{\Gamma_n}^{\Gamma_{n+1}} \norm[2]{\CPE{\int_{\Gamma_n}^s \nabla^2 U(Y_u) \nabla U(Y_u) + (1/2)\vec{\Delta} (\nabla U) (Y_u)\rmd u}{\filtration_{\Gamma_n}} } \rmd s \eqsp.
\end{equation*}
We now separately bound the two last terms of the right hand side.
By \Cref{assum:regularity_2}, the Markov property of $(Y_t)_{t \geq 0}$ and \Cref{lem:moment_diffusion}, we have
\begin{multline}
\label{eq:04/022}
\int_{\Gamma_n}^{\Gamma_{n+1}} \CPE{\norm{  \nabla U(Y_s) - \nabla U(Y_{\Gamma_n})  }^2}{\filtration_{\Gamma_n}} \rmd s %&
%\leq L^2\int_{\Gamma_n}^{\Gamma_{n+1}} \CPE{\norm{Y_s - Y_{\Gamma_n}}^2 }{\filtration_{\Gamma_n}} \rmd s\\
%\label{eq:distance_diffusion_first_part_second_estimate}
%\nonumber
%&
%\qquad \qquad \qquad
\\
 \leq L^2 \left( d \gamma_{n+1}^2 + dL^2 \gamma_{n+1}^4 /12+ (1/2)L^2 \gamma_{n+1}^3 \norm[2]{Y_{\Gamma_n}-x^\star}\right) \eqsp.
\end{multline}
We now bound $A$. We get using Jensen's inequality,  Fubini's theorem, $\nabla U(\xstar) = 0$ and \eqref{eq:borne_Lap_vec}
\begin{align}
\nonumber
A
% &\leq   \int_{\Gamma_n}^{\Gamma_{n+1}} (s - \Gamma_n)\int_{\Gamma_n}^s \CPE{\norm[2]{ \nabla^2 U(Y_u) \nabla U(Y_u) + 2^{-1}\vec{\Delta} (\nabla U) (Y_u)} } {\filtration_{\Gamma_n}}  \rmd u\, \rmd s \\
% \nonumber
 &\leq 2 \int_{\Gamma_n}^{\Gamma_{n+1}} (s - \Gamma_n)\int_{\Gamma_n}^s \CPE{\norm[2]{ \nabla^2 U(Y_u) \nabla U(Y_u) }}{\filtration_{\Gamma_n}}  \rmd  u \, \rmd s \\
\nonumber
 &\phantom{aaaaaaaaa}+  2^{-1} \int_{\Gamma_n}^{\Gamma_{n+1}} (s - \Gamma_n)\int_{\Gamma_n}^s \CPE{\norm[2]{\vec{\Delta} (\nabla U) (Y_u)}}{\filtration_{\Gamma_n}}    \rmd u\, \rmd s\\
\label{eq:04/023}
& \leq 2 \int_{\Gamma_n}^{\Gamma_{n+1}} (s - \Gamma_n) L ^4 \int_{\Gamma_n}^s \CPE{\norm[2]{ Y_u- \xstar} } {\filtration_{\Gamma_n}}\rmd u \, \rmd s  + \gamma_{n+1}^3 d^2 \tilde{L}^2/6  \eqsp.
\end{align}
By \Cref{lem:moment_diffusion}-\ref{item:moment_diffusion_2}, the Markov property and for all $t \geq 0$, $1-\rme^{-t} \leq t$, we have for all $s \in \ccint{\Gamma_n,\Gamma_{n+1}}$,
\begin{equation*}
%  \label{eq:04/024}
  \int_{\Gamma_n}^s \CPE{\norm[2]{ Y_u- \xstar} } {\filtration_{\Gamma_n}}\rmd u \leq
(2m)^{-1}(1-\rme^{-2m(s-\Gamma_n)})\norm[2]{Y_{\Gamma_n}-\xstar} + d(s-\Gamma_n)^2 \eqsp.
\end{equation*}
Using this inequality in \eqref{eq:04/023} and for all $t \geq 0$, $1-\rme^{-t} \leq t$ , we get
\begin{equation*}
A  \leq (2 L^4 \gamma_{n+1}^3/3)\norm[2]{Y_{\Gamma_n}-\xstar} + L^4 d \gamma_{n+1}^4/2 +  \gamma_{n+1}^3 d^2 \tilde{L}^2/6 \eqsp.
\end{equation*}
Combining this bound and \eqref{eq:04/022}   in \eqref{eq:distance_diffusion_part1_first_estimateD} concludes the proof.
\end{proof}



%\begin{proposition}
%\label{propo:distance_interpolate_diffusionD}
%Assume \Cref{assum:regularity_2}, \Cref{assum:potentialU} and \Cref{assum:reg_plus}. Let $(\gamma_k)_{k \geq 1}$ be a non-increasing sequence with $\gamma_1 \leq 1/(m+L)$.
%  Let $\zeta_0 \in \Pens_2(\rset^d \times \rset^d)$, $(Y_t,\overline{Y}_t)_{t \geq 0}$ such that $(Y_0, \overline{Y}_0)$ is distributed according to $\zeta_0$ and
%given by \eqref{eq:definition_couplage_2}.
%Then for all $n \geq 0$ and $t \in \ccint{\Gamma_n , \Gamma_{n+1}}$:
%\begin{equation*}
%\expe{\norm[2]{Y_t - \overlineY_{t}}} \leq u_n^{(1)} (\gamma) \expe{\norm[2]{Y_0 - \overlineY_{0}}} + \tilde{u}^{(4)}_n (\gamma)+ u^{(5)}_{t,n}(\gamma) \eqsp,
%\end{equation*}
%where $(u_n^{(1)}(\gamma))_{n \geq 1}$ is given by \eqref{eq:def_u1}, $ (u_{t,n}^{(5)}(\gamma))_{n \geq 1}$ by \eqref{eq:defu5}, $\delta_i$ by \eqref{eq:defdeltai}  and
%\begin{multline*}
%\widetilde{u}_n^{(4)} (\gamma) \eqdef
%\sum_{i=1}^n d \gamma_{i}^3\parenthese{2L^2+ \kappa^{-1}(\tilde{L}^2/3 + \gamma_{i}L^4) + \gamma_{i}^2 L^4 /6 } \prod_{k=i+1}^n(1- \kappa\gamma_k/2) \\
%+
%L^4 \sum_{i=1}^n  \delta_i  \gamma_{i}^3(4\kappa^{-1}/3+\gamma_{i})  \prod_{k=i+1}^n(1- \kappa \gamma_k/2)
%\end{multline*}
%\end{proposition}
%
%
%\begin{proof}
%The proof is a straightforward adaptation of the one of \Cref{propo:distance_interpolate_diffusion} using \Cref{lem:distance_Euler_diffusion_part1D} instead of \Cref{lem:distance_Euler_diffusion_part1} and is omitted.
%\end{proof}
%\begin{proof}[Proof of \Cref{theo:distance_Euler_diffusionD}]
%The proof is straightforward application of \Cref{propo:distance_interpolate_diffusion}, following the same line as the proof of \Cref{theo:distance_Euler_diffusion}.
%\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> proof_MSE_tv.tex <==
%%Suite proof



% \begin{lemma}
% \label{lem:induction_function_mart_2_tv}
% Assume \Cref{assum:regularity_2} and \Cref{assum:potentialU}. Let $(\gamma_k)_{k \geq 1}$  be a non-increasing sequence
% with $\gamma_1 \leq 2/(m+L)$. Let $N \geq 0$ and $n \geq 1$.
%  Then for all $x \in \rset^d$ and $f \in \functionspace[b]{\rset^d}$,
% \begin{equation*}
% %\label{eq:lem:induction_function_mart_2_tv_1}
% \VarDeux{x}{\martIncF^N_n(X_N)}
% \leq  2 \kappa^{-1} \norm{f}_{\infty}^2 \defEns{ \sum_{i=N+1}^{N+n} \weight{i} /(\uppi \LambdarMSE_{N+1,i})^{1/2} }^2 \eqsp,
%  \end{equation*}
% where $\martIncF_{n}^N$ is given by \eqref{eq:def_F_f} and
% $\LambdarMSE_{N+1,i}$ in \eqref{eq:def_xirmse} for all $i \in
% \{N+1,\cdots,N+n \}$.
% \end{lemma}
% \begin{proof}
% By \eqref{eq:mart_n_0^N_dev} and \Cref{theo:convergence_discrete_chain}-\ref{item:convergence_discrete_chain_3}, $\martIncF_n^N$ is Lipschitz function with
% \begin{align*}
% \norm{\martIncF^N_n}_{\Lip}  \leq   \sum_{i=N+1}^{N+n} \weight{i} \norm{Q_\gamma^{N+1,i}f}_{\Lip} \leq  2 \norm{f}_{\infty} \sum_{i=N+1}^{N+n} \weight{i} /\LambdarMSE^{1/2}_{N+1,i} \eqsp.
% \end{align*}
% Finally, the proof follows from \Cref{lem:var_2}.
% \end{proof}


% \begin{proof}[Proof of \Cref{theo:var_tv}]
%  The proof follows from combining the bounds given by \Cref{lem:induction_function_mart_1_tv} and \Cref{lem:induction_function_mart_2_tv} in \eqref{eq:decomposition-variance-alter}.
% \end{proof}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

